ESCA: Contextualizing Embodied Agents via Scene-Graph Generation

Multi-modal large language models (MLLMs) are making rapid progress toward general-purpose embodied agents. However, existing MLLMs do not reliably capture fine-grained links between low-level visual features and high-level textual semantics, leading to weak grounding and inaccurate perception. To overcome this challenge, we propose ESCA, a framework that contextualizes embodied agents by grounding their perception in spatial-temporal scene graphs. At its core is SGCLIP, a novel, open-domain, promptable foundation model for generating scene graphs that is based on CLIP. SGCLIP is trained on 87K+ open-domain videos using a neurosymbolic pipeline that aligns automatically generated captions with scene graphs produced by the model itself, eliminating the need for human-labeled annotations. We demonstrate that SGCLIP excels in both prompt-based inference and task-specific fine-tuning, achieving state-of-the-art results on scene graph generation and action localization benchmarks. ESCA with SGCLIP improves perception for embodied agents based on both open-source and commercial MLLMs, achieving state of-the-art performance across two embodied environments. Notably, ESCA significantly reduces agent perception errors and enables open-source models to surpass proprietary baselines. We release the source code for SGCLIP model training at https://github.com/video-fm/LASER and for the embodied agent at https://github.com/video-fm/ESCA.

==> figures/app_prompts.tex <==

\begin{minipage}{\textwidth}
\centering
\begin{lstlisting}[language=json, numbers=none, label={app:prompts}]
You will describe the event length and location in 
both natural language and fraction of the video. 
The natural language description of the locations in the video can be: early, mid, late.
The natural language description of the durations of the event can be: long, medium, short
Examples of precise video locations: [1/4, 1/2], [2/3, 1].
Examples of event durations: 1/4, 2/3, 1.


Caption: A man carries a child and walks to the left from behind a woman holding another child.
Video_ID: "0be30efe",
Action json: 
{"video_id": "0be30efe", 
 "sequential descriptions": [ "man A carry child B, women C hold child D, man A is behind women C", "man A walk", "man A at left" ], 
  "time stamps": 
    { "1": { "description": [ "man A carry child B", "women C hold child D", "man A is behind women C" ], "programmatic": [ "carrying(A, B)", "name(A, man)", "name(B, child)", "holding(C, D)", "name(C, women)", "name(D, man)", "behind(A, C)",  ], "duration": "short", "duration precise": "1/4", "video location": "early",  "video location precise": "[0, 1/4]" }, "2": { "description": [ "man A walk" ], "programmatic": [ "walk(A)", ], "duration": "medium", "duration precise": "1/2", "video location": "mid", "video location precise": "[1/4, 3/4]" }, "3": { "description": [ "man A at left" ], "programmatic": [ "left(A)" ], "duration": "short", "duration precise": "1/4", "video location": "late", "video location precise": "[3/4, 1]"}}}


Caption: "A woman is teasing a kitten with a piece of meat, and the kitten is peeking its head from a chair to look at the meat."
Video_id: "0010_86102",
Action json: { "video_id": "0010_86102", "sequential descriptions": [ "woman A teasing kitten B with meat C", "kitten B peek at meat C from a chair D", ], "time stamps": { "1": {"description": [ "woman A teasing kitten B with meat C", ], "programmatic": [ "sitting on(B, D)", "name(B, cat)", "name(D, chair)", "name(A, adult)", "name(C, meat)" ], "duration": "mid", "duration precise": "1/2", "video location": "early", "video location precise": "[0, 1/2]" }, "2": { "description": [ "kitten B peek at meat C from a chair D" ], "programmatic": [ "catching(B, C)", "sitting on(B, D)" ], "duration": "long", "duration precise": "1", "video location": "mid", "video location precise": "[0, 1]"}}}
\end{lstlisting}
\end{minipage}



\begin{minipage}{\textwidth}
\centering
\begin{lstlisting}[language=json, numbers=none]
Caption: "The young boy receives another gift and sits on the floor."
Video_id: "03f2ed96-1719",
Action json: {"video_id": "03f2ed96-1719","sequential descriptions": ["boy A receives gift B", "boy A sits on the floor C"], "time stamps": {"1": { "description": ["boy A receives gift B",], "programmatic": ["holding(B, D)", "name(A, boy)", "name(B, gift)",], "duration": "mid","duration precise": "1/2","video location": "early", "video location precise":  "[0, 1/2]"}, "2": { "description": [ "boy A sits on the floor C",], "programmatic": ["sitting on(A, C)", "name(A, boy)", "name(C, floor)", ], "duration": "mid", "duration precise": "1/2", "video location": "late", "video location precise": "[1/2, 1]"}}}


Note all the relations are name, unary or binary.
A name relation takes in two arguments, the first is always a variable, and the second argument could be noun ("apple"), noun phrase ("ancient_building"), location("dark_forest"), etc. For example "name(A, "apple")" means the variable A refers to an apple. Please ensure no space occur in the second argument.
A unary relation takes in one variable as its argument. For example, close(A) means A is close to the camera.
A binary relation takes in two variables as its arguments. For example, above(A, B) means A is above B.
The entity in the binary and unary relation are variables in the form of capitalized letters (A, B).
The predicate of the unary relation can be adjectives, verbs, and name.
The predicate of the binary relation can be preposition, and verb. 
Please include the name relation any time if applicable.
Please make the preposition and adjectives into separate two relation. 
For each time stamp, please only describe the events that are happening at the same time, if any sequential events occur, put them into multiple time stamps. 
For example, instead of 'person A enter from left, person A walk to center, person A move to couch' in one time stamp, 
put it into three different time stamps: "person A enter from left", "person A walk to center", "person A move to couch".
Please only describe one single event in sequential description per time stamp. 
Please use as many relations as possible to precisely describe the action.
Please generate the action json programs for the following captions in the following format:
{"actions": {caption_id: action json programs}}
IMPORTANT: Please REMOVE all new line characters and extra spaces in the generated json!

\end{lstlisting}
\end{minipage}



==> figures/performance-eb-habitat.tex <==
\begin{table}[t]
    \centering
    \small
    \begin{tabular}{llrrrrrrr}
        \toprule
        \multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\textbf{Strategy}} & \multicolumn{6}{c}{\textbf{Subset}} & \multirow{2}{*}{\textbf{Avg}} \\ \cmidrule{3-8}
            &  & Base & Common & Complex & Visual & Spatial & Long & \\
        \midrule
        \multirow{3}{*}{InternVL-2.5-38B-MPO} 
            & Base      & 92.00 & 24.00 & 64.00 & 46.00 & 30.00 & 32.00 & 48.00 \\
            & + GD      & 84.00 & 36.00 & 66.00 & 52.00 & 32.00 & 40.00 & 51.67 \\
            & + \ours   & 94.00 & 46.00 & 62.00 & 54.00 & 34.00 & 40.00 & \textbf{55.00} \\
        \midrule
        \multirow{3}{*}{Gemini-2.0-flash} 
            & Base      & 66.00 & 20.00 & 32.00 & 32.00 & 20.04 & 10.20 & 30.04 \\
            & + GD      & 68.00 & 18.36 & 32.00 & 24.00 & 20.41 & 10.00 & 28.80 \\
            & + \ours   & 74.00 & 22.00 & 35.14 & 36.00 & 22.00 & 14.00 & \textbf{33.86} \\
        \midrule
        \multirow{3}{*}{Qwen2.5-VL-72B-Ins} 
            & Base      & 58.00 & 18.00 & 42.00 & 40.00 & 24.00 & 18.00 & 33.33 \\
            & + GD      & 52.00 & 50.00 & 68.00 & 70.00 & 21.00 & 36.00 & 49.50 \\
            & + \ours   & 86.00 & 50.00 & 72.00 & 60.00 & 36.00 & 34.00 & \textbf{56.33} \\
        \midrule
        \multirow{3}{*}{GPT-4o} 
            & Base      & 86.00 & 44.00 & 56.00 & 68.00 & 36.00 & 64.00 & 59.00 \\
            & + GD      & 92.00 & 46.00 & 52.00 & 66.00 & 34.00 & 60.00 & 58.33 \\
            & + \ours   & 92.00 & 52.00 & 68.00 & 68.00 & 32.00 & 52.00 & \textbf{60.67} \\
        \bottomrule
    \end{tabular}
    \vspace{5px}
    \caption{Detailed performance on EB-Habitat, decomposed by subsets of tasks.}
    \label{tab:grounding-strategies-hab}
\end{table}



